Which Student is Best? A Comprehensive Knowledge Distillation Exam for Task-Specific BERT Models

We perform knowledge distillation (KD) benchmark from task-specific BERT-base teacher models to various student models: BiLSTM, CNN, BERT-Tiny, BERT-Mini, and BERT-Small. Our experiment involves 12 datasets grouped in two tasks: text classification and sequence labeling in the Indonesian language. We also compare various aspects of distillations including the usage of word embeddings and unlabeled data augmentation. Our experiments show that, despite the rising popularity of Transformer-based models, using BiLSTM and CNN student models provide the best trade-off between performance and computational resource (CPU, RAM, and storage) compared to pruned BERT models. We further propose some quick wins on performing KD to produce small NLP models via efficient KD training mechanisms involving simple choices of loss functions, word embeddings, and unlabeled data preparation.

==> sec-res-old.tex <==
Across the board, the BERT-base teacher model outperforms the other models, which we discuss thoroughly below. We first focus on the models' performance in terms of F1 score (see Table~\ref{tbl-cls} and Table~\ref{tbl-seqlab} for the complete results of classification and sequence labeling tasks, respectively). Then, we discuss the models' cost analysis in terms of their size and inference time (Table~\ref{tbl-cost} and Table~\ref{tbl-onnx}.

\begin{table*}[]
\caption{Classification KD}
\label{tbl-cls}
\begin{tabular}{lrrrrrrr}
\toprule
\multicolumn{1}{c}{Models} & \multicolumn{1}{c}{Smltk} & \multicolumn{1}{c}{Health} & \multicolumn{1}{c}{Telco} & \multicolumn{1}{c}{SentA} & \multicolumn{1}{c}{EmoT} & \multicolumn{1}{c}{SMSA} & \multicolumn{1}{c}{avg} \\ \midrule
BERT              & 96.83 & 80.01 & 94.96 & 90.01 & 72.30 & 91.49 & 87.60 \\ \midrule
Bi-LSTM           & 86.78 & 72.22 & 88.16 & 76.35 & 55.96 & 83.84 & 77.22 \\
KD                & 92.96 & 74.25 & 91.41 & 82.28 & 66.72 & 88.67 & 82.72 \\
KD Ulb            & 92.74 & 77.61 & 92.71 & 85.17 & 68.33 & 88.81 & 84.23 \\ 
KD Ulb + FastText & 93.03 & 77.97 & 92.57 & 85.80 & 69.40 & 88.34 & 84.52 \\
KD Ulb + BERT Embed & 92.79 & 78.78 & 92.15 & 86.28 & 69.54 & 88.77 & 84.72 \\
\midrule
CNN               & 88.24 & 71.97 & 88.22 & 77.95 & 57.57 & 84.12 & 78.01 \\
KD            & 92.43 & 69.85 & 90.95 & 80.33 & 63.90 & 87.26 & 80.79 \\
KD Ulb        & 84.50 & 74.32 & 84.05 & 82.46 & 63.92 & 87.75 & 79.50 \\  
KD Ulb + FastText & 81.23 & 73.27 & 86.40 & 84.65 & 65.97 & 88.44 & 79.99 \\
KD Ulb + BERT Embed & 85.35 & 74.20 & 86.72 & 84.01 & 64.48 & 87.40 & 80.36 \\
\midrule 
BERT-Tiny & 89.89 & 69.46 & 86.31 & 77.36 & 60.42 & 79.88 & 77.22 \\
KD & 91.87 & 76.27 & 90.05 & 81.56 & 67.10 & 83.79 & 81.77 \\
KD Ulb & 94.02 & 77.74 & 92.17 & 83.06 & 66.21 & 86.39 & 83.26 \\
KD Ulb + FastText & 94.48 & 78.32 & 92.40 & 82.52 & 66.97 & 86.90 & 83.60 \\
KD Ulb + BERT Embed & 95.31 & 77.02 & 92.69 & 83.17 & 66.90 & 86.28 & 83.56 \\
\midrule
BERT-Mini & 91.62 & 68.88 & 89.70 & 80.47 & 60.27 & 81.93 & 78.81 \\
KD & 94.40 & 77.95 & 92.96 & 81.78 & 68.26 & 86.81 & 83.69 \\
KD Ulb & 95.10 & 77.87 & 93.43 & 83.57 & 69.62 & 85.02 & 84.10 \\
KD Ulb + FastText & 96.37 & 77.93 & 93.72 & 83.95 & 68.87 & 86.10 & 84.49 \\
KD Ulb + BERT Embed & 95.73 & 77.95 & 94.22 & 81.95 & 69.75 & 87.99 & 84.60 \\
\midrule
BERT-Small        & 92.92 & 73.81 & 91.35 & 80.20 & 62.65 & 83.77 & 80.78 \\
KD     & 94.74 & 78.82 & 92.69 & 80.78 & 69.01 & 87.21 & 83.88 \\
KD Ulb & 96.51 & 78.73 & 94.18 & 83.90 & 69.60 & 87.51 & 85.07 \\  
KD Ulb + FastText & 96.38 & 77.94 & 94.25 & 82.43 & 69.83 & 87.85 & 84.78 \\
KD Ulb + BERT Embed & 96.30 & 77.95 & 94.54 & 85.16 & 70.53 & 88.32 & 85.47 \\
\bottomrule
\end{tabular}
\end{table*}

%\subsubsection{Vanilla vs KD}



% We first run the baseline, the BERT model as the teacher that we want to achieve and the student models, Bi-LSTM, CNN, and BERT-Small. We could see that BERT outperform every student models. Based on baseline student model, BERT-Small gave the best result. As our BERT-Small model was trained from scratch without prior pre-training knowledge, it shows that BERT's architecture strongly contribute to the improvement of the models's performance in compare to the older Deep Learning models.

Every student models gain improvement after training with KD, showing the efficientcy of the methods. Amongst all student models, Bi-LSTM get the most gain with 5.5 point improvement and almost as good as BERT-Small with KD. If we consider model's size (see Table~\ref{tbl-cost}), this method can be more appealing.

- Compare base Bi-LSTM vs CNN vs Bert-SMALL
- Compare the KD of them

\subsubsection{Unlabelled Data Classification}
\label{sec-ulb-class}

In this experiment, we simply combined the unique training data from all dataset. By doing this, we also want to now the effect of adding out-of-domain data to KD's performance.
The total unlabelled data that we use for this experiment is 74688. In average, adding more data, although out-of-domain, increase the overall performance. It can be expected as KD only learn to be as similar as the teacher as possible with no regard to the original label. The affect of adding more data can be shown to be the best for BERT-Small. It was expected as BERT architect need a lot of training data. 

It was interesting that in CNN, addding unlabelled that can worsen the final performance. We assumed that adding many unlabelled data meant no control in data cleanliness and could create imbalance, thus resulting in a worse performance. 
Further exploration to investigate why this happened can be seen on Section~\ref{sec-discuss}.
 
\subsection{Experiment on Sequence Labeling}

Next, we tried to explore several methods for sequence labeling task. The full results can be seen on Table~\ref{tbl-seqlab}.

\begin{table*}[]
\caption{Sequence Labelling KD}
\label{tbl-seqlab}
\begin{tabular}{lrrrrrrr}
\toprule
\multicolumn{1}{c}{Models} & \multicolumn{1}{c}{EntK} & \multicolumn{1}{c}{TermA} & \multicolumn{1}{c}{POS} & \multicolumn{1}{c}{NERGrit} & \multicolumn{1}{c}{NERP} & \multicolumn{1}{c}{POSP} & \multicolumn{1}{c}{avg} \\ \midrule
BERT                & 90.86 & 90.38 & 95.66 & 75.78 & 78.35 & 95.81 & 87.81 \\ \midrule
BiLSTM              & 79.21 & 84.38 & 91.12 & 44.00 & 58.56 & 93.59 & 75.14 \\
KD MSE Loss         & 83.32 & 87.13 & 93.05 & 52.56 & 66.88 & 94.95 & 79.65 \\
KD KLD Loss         & 85.99 & 88.08 & 93.56 & 56.80 & 69.10 & 95.05 & 81.43 \\
KD Ulb              & 86.24 & 87.82 & 94.11 & 62.90 & 70.38 & 95.57 & 82.84 \\
KD Ulb + FastText   & 86.50 & 88.15 & 94.29 & 66.52 & 72.27 & 95.70 & 83.91 \\
KD Ulb + BERT Embed & 86.28 & 88.22 & 94.44 & 68.26 & 72.40 & 95.77 & 84.23  \\ \midrule
CNN                 & 80.17 & 84.70 & 91.94 & 39.86 & 59.52 & 94.45 & 75.11 \\
KD MSE Loss         & 87.41 & 88.63 & 93.97 & 60.10 & 71.14 & 94.95 & 82.70 \\
KD KLD Loss         & 86.26 & 88.83 & 93.70 & 60.43 & 70.78 & 95.40 & 82.57 \\
KD Ulb              & 87.91 & 89.11 & 94.49 & 70.28 & 73.33 & 95.87 & 85.17 \\
KD Ulb + FastText   & 87.47 & 88.06 & 94.40 & 69.17 & 72.24 & 95.67 & 84.50  \\
KD Ulb + BERT Embed & 88.60 & 89.22 & 94.42 & 68.88 & 73.62 & 95.64 & 85.06 \\ 
\midrule 
BERT-Tiny & 67.53 & 78.60 & 89.83 & 34.06 & 48.14 & 93.02 & 68.53 \\
KD MSE Loss & 83.32 & 87.54 & 92.82 & 47.83 & 68.21 & 93.97 & 78.95 \\
KD KLD Loss & 78.24 & 84.82 & 92.02 & 34.63 & 65.58 & 93.62 & 74.82\\
KD Ulb & 86.38 & 87.21 & 94.56 & 64.65 & 71.87 & 95.37 & 83.34 \\
KD Ulb + FastText & 86.33 & 87.60 & 94.16 & 64.02 & 70.59 & 95.12 & 82.97 \\
KD Ulb + BERT Embed & 86.49 & 87.80 & 94.44 & 65.51 & 71.39 & 95.54 & 83.53 \\
\midrule
BERT-Mini & 72.10 & 79.97 & 90.95 & 34.89 & 56.69 & 93.05 & 71.27 \\
KD MSE Lossi & 88.41 & 88.62 & 94.21 & 55.59 & 72.78 & 95.38 & 82.50 \\
KD KLD Loss & 83.04 & 85.98 & 92.22 & 51.91 & 67.65 & 94.22 & 79.17 \\
KD Ulb & 89.69 & 89.01 & 95.15 & 70.48 & 75.24 & 95.87 & 85.91 \\
KD Ulb + FastText & 89.86 & 89.34 & 95.28 & 70.73 & 75.31 & 95.95 & 86.08 \\
KD Ulb + BERT Embed & 90.20 & 89.14 & 95.23 & 71.72 & 76.16 & 96.05 & 86.42 \\
\midrule
BERT-Small          & 75.89 & 79.77 & 90.66 & 32.87 & 54.48 & 93.28 & 71.16 \\
KD MSE Loss         & 88.27 & 88.33 & 94.18 & 60.37 & 72.05 & 95.14 & 83.06 \\
KD KLD Loss         & 84.16 & 86.92 & 93.02 & 55.06 & 69.09 & 94.70 & 80.49 \\
KD Ulb              & 89.65 & 88.82 & 95.21 & 71.11 & 75.20 & 95.87 & 85.98 \\
KD Ulb + FastText   & 89.36 & 88.70 & 95.37 & 70.86 & 75.96 & 96.02 & 86.04 \\
KD Ulb + BERT Embed & 90.44 & 88.89 & 95.32 & 71.54 & 76.08 & 96.05 & 86.39 \\ 
\bottomrule
\end{tabular}
\end{table*}

\subsubsection{Vanilla vs KD MSE vs KD KLD }

Like previous work, we run the model to the Teacher and Student with no KD to get the goal that we want to achive and the starting point. Unlike text classification, in sequence labeling, BERT-Small from scratch performed the worst amongst all student models while BiLSTM and CNN performance are similar.

Next, we tried to apply KD. In sequence labeling task, we compare two different loss function: MSE and KLD as several previous works use KLD for their loss function when they work on sequence labeling data. In general, using KD improve the overall performance no matter what loss function that we use. Between MSE and KLD, we found that it depends on the algorithms itself in which loss function would gave better result. In BiLSTM, using KLD is always better than MSE, but in BERT-Small, MSE always outperform KLD. In CNN, several dataset performed better when using MSE while others using KLD is better, but the overall performance show that MSE is better. Because of the difference in result, in the next step, for each model we use its best previous result.

- Compare with classification about the bert small (hgihest in classification, yet bad in seqlab)


\subsubsection{Unlabelled Data Sequence Labeling}

We use the same method as we described in Section~\ref{sec-ulb-class} to generate the data.
For sequence labeling task, the total amount of unlabelled data is 30130. 

In this task, adding more data always improve the performance except for TermA with Bi-LSTM model. We assumed it probably because TermA has a domain specific data and labels (hotel review) while the other use general data and label. Thus adding more data, although come from different domain, would overall give more benefits. In average adding unlabelled data would give 2.3 points of improvement. Similar to text classification task, BERT-Small gave the most gain, further confirming that BERT architecture would benefit with more training data.

\subsubsection{Embedding}

We want to explore the effect of initializing Embedding with pre-trained embedding. As for BERT-Small, as its embedding size (512) is larger than FastText (300), we only experiment with BERT Embedding.

In average, adding pre-trained embedding would give some improvements to the overall result. Other than that, it also speed up training into convergence (see Appendix Figure~\ref{fig:train-converge-embed}).

\subsection{Cost Analysis}

To give a deeper analysis, we compare model size and its inference time that can gave a prediction on the cost of deploying each model. See table~\ref{tbl-cost} for detail.

\begin{table}[width=.9\linewidth,cols=5,pos=h]
\caption{Model Size and Inference time comparison. Model size is in number of million (M) of parameters. Inference Time for both GPU and CPU in miliseconds (ms).}
\label{tbl-cost}
\begin{tabular}{lrrr}
\toprule
\multicolumn{1}{c}{Model} & \multicolumn{1}{c}{Param} & \multicolumn{1}{c}{CPU} & \multicolumn{1}{c}{GPU} \\ \midrule
\multicolumn{4}{c}{Classification} \\ \midrule
BERT & 124.51 & 39.15 & 11.69 \\
Bi-LSTM & 3.35 & 1.74 & 1.09 \\
CNN & 4.02 & 2.36 & 2.96 \\
BERT-Tiny & 4.40 & 2.07 & 2.47 \\
BERT-Mini & 11.19 & 4.52 & 4.21 \\
BERT-Small & 28.81 & 8.93 & 4.28 \\ 
\midrule
\multicolumn{4}{c}{Sequence Labeling} \\ \midrule
BERT & 124.46 & 67.18 & 12.43 \\
Bi-LSTM & 4.38 & 3.19 & 1.61 \\
CNN & 4.01 & 2.35 & 3.12 \\
BERT-Tiny & 4,40 & 2.24 & 2.46 \\
BERT-Mini & 11.18 & 6.32 & 4.48\\
BERT-Small & 28.78 & 9.25 & 4.50 \\ 
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Model Size}

In average, older deep learning model like Bi-LSTM and CNN are 31x smaller with only 3-4 point difference.
If we still want to use BERT's strong architecture, we could use a smaller size bert such as BERT-Small. With only 1-2 point difference, it was only 23\% the size of the original BERT model. While sacrificing slight loss, these models is more feasible to be deployed for production.

\subsubsection{Inference time}

For deep neural model, using GPU can speed up the inference time. An exception occurred in convolutional models that used depthwise separable convolution operations (like our CNN models), the decreasing speed is an ongoing issue related to the CUDA library\footnote{https://github.com/pytorch/pytorch/issues/18631}.  If have a unlimited amount of GPU or only need to serve a few models, the time for inference is not too bad. However, it often becomes infeasible for production environment as we need to host multiple models. It could also become a problem when we want to scale our products.

\subsubsection{Using ONNX}

ONNX is a cross-platform inferencing and training accelerator compatible with popular ML/DNN frameworks, including PyTorch, TensorFlow/Keras, scikit-learn, and more (ref). The idea of ONNX Runtime is similar to JVM, to tackle interpretability (ref). It could be executed in different runtime environments and doesn’t need to package every dependency. However it’s still a new technology that sometimes often faces issues. 

ONNX Runtime has shown to speed the model inference time running in the CPU machine (ref, ref). As it is infeasible to provide a GPU machine for production environment, we try to use this technology to speed inference time using CPU. Converting the model to ONNX also shown to remove PyTorch library dependency, which result in a smaller image size when we create a docker service. 

original model size. In some cases, it even results in only 30\% of the original model’s size. This shows that saving the model in onnx format would save storage space for neural models.

\begin{table}[width=.9\linewidth,cols=5,pos=h]
\caption{onnx. Model size in according to its file size in MB and inference time using CPU in ms.}
\label{tbl-onnx}
\begin{tabular}{lrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{ONNX} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Size} & \multicolumn{1}{c}{CPU} & \multicolumn{1}{c}{Size} & \multicolumn{1}{c}{CPU} \\ \midrule
\multicolumn{5}{c}{Classification} \\
\midrule
BERT &  1425.17 & 39.15 & 475.06 & 46.72 \\
Bi-LSTM & 38.40 & 1.74 & 12.80 & 0.36 \\
CNN & 46.06 & 2.36 \\
BERT-Tiny & 50.38 & 2.07 & 16.79 & 0.30 \\
BERT-Mini & 128.20 & 4.52 & 42.73 & 1.78 \\
BERT-Small & 329.81 & 8.93 & 109.94 & 7.25 \\ 
\midrule
\multicolumn{5}{c}{Sequence Labeling} \\
\midrule
BERT & \\
Bi-LSTM & \\
CNN & \\
BERT-Tiny & \\
BERT-Mini & \\
BERT-Small & \\
\bottomrule
\end{tabular}
\end{table}

